Inference for Large-Scale Linear Systems with Known Coefficients

This paper considers the problem of testing whether there exists a non-negative solution to a possibly under-determined system of linear equations with known coefficients. This hypothesis testing problem arises naturally in a number of settings, including random coefficient, treatment effect, and discrete choice models, as well as a class of linear programming problems. As a first contribution, we obtain a novel geometric characterization of the null hypothesis in terms of identified parameters satisfying an infinite set of inequality restrictions. Using this characterization, we devise a test that requires solving only linear programs for its implementation, and thus remains computationally feasible in the high-dimensional applications that motivate our analysis. The asymptotic size of the proposed test is shown to equal at most the nominal level uniformly over a large class of distributions that permits the number of linear equations to grow with the sample size.

==> figures-and-tables/size_table_lb_5-auto.tex <==
\begin{tabular}{@{}c c cc c cc c cc c cc c cc c cc c c@{}}
	\toprule
	 &  & \multicolumn{7}{c}{$d$} \\
	\cmidrule(lr){3-9}
	$n$ & $p$ & 100 & 400 & 1600 & 4900 & $100^{2}$ & $225^{2}$ & $317^{2}$ \\
	\midrule
	\multirow{2}{*}{1000} & 6 & .036 & .034 & .034 & .037 & .038 & .036 & .036 \\
	 & 18 & .040 & .035 & .036 & .041 & .039 & .038 & .036 \\
	\cmidrule(lr){1-9}
	\multirow{3}{*}{2000} & 6 & .042 & .042 & .049 & .046 & .047 & .052 & .061 \\
	 & 18 & .031 & .028 & .032 & .032 & .030 & .030 & .028 \\
	 & 38 & .053 & .046 & .051 & .052 & .052 & .067 & .053 \\
	\cmidrule(lr){1-9}
	\multirow{4}{*}{4000} & 6 & .045 & .048 & .049 & .054 & .058 & .051 & .065 \\
	 & 18 & .028 & .031 & .029 & .028 & .030 & .038 & .035 \\
	 & 38 & .031 & .034 & .039 & .036 & .040 & .035 & .037 \\
	 & 51 & .042 & .051 & .051 & .040 & .047 & .047 & .030 \\
	\cmidrule(lr){1-9}
	\multirow{5}{*}{8000} & 6 & .049 & .055 & .056 & .048 & .054 & .055 & .073 \\
	 & 18 & .034 & .035 & .036 & .030 & .032 & .040 & .041 \\
	 & 38 & .033 & .035 & .035 & .037 & .037 & .025 & .047 \\
	 & 51 & .034 & .043 & .035 & .040 & .037 & .035 & .038 \\
	 & 83 & .043 & .042 & .050 & .048 & .042 & .054 & .046 \\
	\bottomrule
\end{tabular}


==> figures-and-tables/size_table_lb_5-mult.tex <==
\begin{tabular}{@{}c c cc c cc c cc c cc c cc c cc c c@{}}
	\toprule
	 &  & \multicolumn{7}{c}{$d$} \\
	\cmidrule(lr){3-9}
	$n$ & $p$ & 100 & 400 & 1600 & 4900 & $100^{2}$ & $225^{2}$ & $317^{2}$ \\
	\midrule
	\multirow{2}{*}{1000} & 6 & .020 & .019 & .021 & .021 & .022 & .019 & .021 \\
	 & 18 & .037 & .029 & .029 & .033 & .033 & .031 & .030 \\
	\cmidrule(lr){1-9}
	\multirow{3}{*}{2000} & 6 & .030 & .025 & .033 & .032 & .033 & .027 & .039 \\
	 & 18 & .023 & .021 & .028 & .027 & .025 & .027 & .020 \\
	 & 38 & .048 & .039 & .043 & .045 & .047 & .062 & .046 \\
	\cmidrule(lr){1-9}
	\multirow{4}{*}{4000} & 6 & .034 & .034 & .038 & .042 & .046 & .035 & .058 \\
	 & 18 & .023 & .026 & .024 & .022 & .025 & .032 & .028 \\
	 & 38 & .026 & .029 & .033 & .032 & .035 & .032 & .033 \\
	 & 51 & .038 & .044 & .045 & .034 & .042 & .041 & .027 \\
	\cmidrule(lr){1-9}
	\multirow{5}{*}{8000} & 6 & .040 & .046 & .048 & .040 & .046 & .050 & .061 \\
	 & 18 & .028 & .028 & .032 & .025 & .027 & .032 & .034 \\
	 & 38 & .027 & .029 & .030 & .032 & .032 & .021 & .043 \\
	 & 51 & .029 & .036 & .028 & .034 & .033 & .030 & .031 \\
	 & 83 & .038 & .035 & .046 & .041 & .034 & .048 & .042 \\
	\bottomrule
\end{tabular}

